Stochastic Load Balancing with Machine Reservations

We introduce a novel variant of stochastic load balancing that enables a quantitative tradeoff between the practical benefits of non-adaptive policies and their performance limitations. Our model describes a solution in two stages. In the first stage, given only job-size distributions, we reserve a set of at most k machines for each job (a k-reservation). In the second stage, after observing job-size realizations, we assign each job to one of its reserved machines (a consistent assignment). The goal is to minimize the expected makespan. If k=1, we get the standard stochastic load balancing problem of finding a non-adaptive assignment with minimum expected makespan. If k is equal to the number of machines, then we obtain an all-powerful omniscient optimum that can tailor the assignment arbitrarily to the job-size realizations. We give a number of results that quantify this tradeoff. Most saliently, we show that in the setting of identical machines, a 2-reservation suffices to achieve a constant-factor approximation to the omniscient optimum, establishing a "power-of-two-choices" result for stochastic load balancing. We also show that this no longer holds true in the more challenging setting of related machines. Nonetheless, we give a number of positive algorithmic results for this setting: a true O(log m/log log m)-approximation; a bicriteria O(1)-approximation by reserving twice as many machines per job relative to an optimal k-reservation; and a 2-reservation whose cost is within a constant factor of what the adaptive optimum can achieve.

==> arxiv_macros.tex <==
\usepackage{times}
\usepackage{xspace}
\usepackage{array} 
\usepackage{amsthm}

\usepackage[dvipsnames]{xcolor}
\usepackage{bbm}
\usepackage[shortlabels,inline]{enumitem}
\usepackage{amsmath,amsthm,amsfonts,amstext,amssymb}
\usepackage[margin=1cm]{caption}
\usepackage[T1]{fontenc}
% \usepackage{newtxtext}
\usepackage{lmodern}
\usepackage[mathscr]{euscript}
\RequirePackage{doi}
\usepackage{hyperref}
\usepackage{slantsc}
\usepackage{comment}
\hypersetup{colorlinks = true,linkcolor = blue, anchorcolor = blue, citecolor = blue, filecolor = red,urlcolor = blue, breaklinks=true}


\usepackage{tikz}
\usetikzlibrary{patterns,decorations.pathreplacing}

% \usepackage{cleveref}

\usepackage[shortcuts]{extdash}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{suffix}
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}
\usepackage{xspace}
\usepackage{comment}
\usepackage{mathtools}
\usepackage[sans]{dsfont} 
% \usepackage{thm-restate} % restatable theorems and lemmas  
\usepackage[shortlabels,inline]{enumitem}
\setlist[enumerate]{font=\normalfont}

\usepackage{hyperref}

\hypersetup{
    colorlinks=true,
    linkcolor=violet,
    filecolor=magenta,      
    urlcolor=cyan,
    citecolor=blue,
    pdffitwindow=true,
}

\usepackage[nameinlink,capitalise]{cleveref} % auto inferring of theorem/lemma based on label

\usepackage{thm-restate} % restatable theorems and lemmas  

% \interfootnotelinepenalty=10000

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}

%% some templates don't have a qed symbol. Custom command to print the symbol only when needed. Prevents double printing.  
% \newcommand{\customqed}{}

\newenvironment{proofof}[1]{%
  \begin{proof}[{Proof of #1}]%
}{%
  \end{proof}%
}
